An investigation of challenges encountered when specifying training data and runtime monitors for safety critical ML applications

Context and motivation: The development and operation of critical software that contains machine learning (ML) models requires diligence and established processes. Especially the training data used during the development of ML models have major influences on the later behaviour of the system. Runtime monitors are used to provide guarantees for that behaviour. Question / problem: We see major uncertainty in how to specify training data and runtime monitoring for critical ML models and by this specifying the final functionality of the system. In this interview-based study we investigate the underlying challenges for these difficulties. Principal ideas/results: Based on ten interviews with practitioners who develop ML models for critical applications in the automotive and telecommunication sector, we identified 17 underlying challenges in 6 challenge groups that relate to the challenge of specifying training data and runtime monitoring. Contribution: The article provides a list of the identified underlying challenges related to the difficulties practitioners experience when specifying training data and runtime monitoring for ML models. Furthermore, interconnection between the challenges were found and based on these connections recommendation proposed to overcome the root causes for the challenges.

==> 2022 - Runtime monitoring VEDLIoT/macro-editing.tex <==
\usepackage{ifthen}
\usepackage{amssymb}
\newboolean{showcomments}
\setboolean{showcomments}{true} % toggle to show or hide comments and proof reading markings


\ifthenelse{\boolean{showcomments}}
  {\newcommand{\nb}[2]{
    \fcolorbox{gray}{yellow}{\bfseries\sffamily\scriptsize#1}
    {\sf\small$\blacktriangleright$\textit{#2}$\blacktriangleleft$}
   }
   \newcommand{\version}{\emph{\scriptsize$-$working$-$}}
  }
  {\newcommand{\nb}[2]{}
   \newcommand{\version}{}
  }

\newcommand\martin[1]{\nb{Hans-Martin}{#1}}
\newcommand\eric[1]{\nb{Eric}{#1}}
\newcommand\jennifer[1]{\nb{Jennifer}{#1}}
\newcommand\padmini[1]{\nb{Padmini}{#1}}
\newcommand\olof[1]{\nb{Olof}{#1}}
\newcommand\oliver[1]{\nb{Oliver}{#1}}
\newcommand\stefan[1]{\nb{Stefan}{#1}}

% Macros for proof-reading
\usepackage[normalem]{ulem} % for \sout
\usepackage{xcolor}

\ifthenelse{\boolean{showcomments}}
  {
  \newcommand{\ra}{$\rightarrow$}
  \newcommand{\ugh}[1]{\textcolor{red}{\uwave{#1}}} % please rephrase
  \newcommand{\ins}[1]{\textcolor{blue}{\uline{#1}}} % please insert
  \newcommand{\del}[1]{\textcolor{red}{\sout{#1}}} % please delete
  \newcommand{\chg}[2]{\textcolor{red}{\sout{#1}}{\ra}\textcolor{blue}{\uline{#2}}} % please change
  \newcommand{\inspar}[1]{\color{blue}{#1}\color{blue}} % Put edit comments in a really ugly standout display
  }
  {
  \newcommand{\ra}{}
  \newcommand{\ugh}[1]{#1} % Keeps original
  \newcommand{\ins}[1]{#1} % Inserts text
  \newcommand{\del}[1]{} % Removes text
  \newcommand{\chg}[2]{#2} % Keeps only the proposed change
  \newcommand{\inspar}[1]{} % Removes edit and box
  
  }

==> 2022 - Runtime monitoring VEDLIoT/nice_tables.tex <==
%% Nice Tables
\usepackage{booktabs}
\usepackage{array}
\usepackage{colortbl}
\usepackage{multirow}
\usepackage{longtable}


\newcolumntype{v}[1]{>{\raggedright \hspace {0pt}}p{#1}}

==> 2022 - Runtime monitoring VEDLIoT/tab_conv_new.tex <==
\begin{table*}[!t]
\centering
\scriptsize
\caption{Challenge groups (bold) and themes found in the interview data. Data.: Challenges related to specifying training data (RQ1). Monitor.: Challenges related to specifying runtime monitoring (RQ2).}
\label{tab:themes}
\begin{tabular}{clccc}
\hline
\multicolumn{1}{c}{}                              & \multicolumn{1}{c}{}                                           & \multicolumn{2}{c}{\textbf{Relates to}} & \multicolumn{1}{c}{\textbf{Related}}                               \\
\multicolumn{1}{c}{\multirow{-2}{*}{\textbf{ID}}} & \multicolumn{1}{c}{\multirow{-2}{*}{\textbf{Challenge Theme}}} & \multicolumn{1}{c}{\textbf{Data.}} & \multicolumn{1}{c}{\textbf{Monitor.}} & \multicolumn{1}{c}{\textbf{Literature}} \\ \hline
\rowcolor[HTML]{EFEFEF} 
\textbf{1}                                        & \textbf{Lack of explainability about ML decisions}             & \textbf{}                         & \textbf{\checkmark} &                        \\
\rowcolor[HTML]{EFEFEF} 
1.1                                               & No access to inner states of ML models                         &                               & \checkmark  &  [18]                            \\
\rowcolor[HTML]{EFEFEF} 
1.2                                               & No failure models for ML models                                &                                   & \checkmark &    [51]                             \\
\rowcolor[HTML]{EFEFEF} 
1.3                                               & IP protection                                                  &                                   & \checkmark &                                \\
\textbf{2}                                       & \textbf{Missing conditions for runtime checks}                 & \textbf{}                         & \textbf{\checkmark} &                       \\
2.1                                              & Unclear metrics and/or boundary conditions          &                                   & \checkmark  & [11,21,43]                              \\
2.2                                              & Unclear measure of confidence                                  &                                   & \checkmark & [17,34]                                \\
\rowcolor[HTML]{EFEFEF} 
\textbf{3}                                      & \textbf{Missing guidelines for data selection}                 & \textbf{\checkmark}                        & \textbf{\checkmark}   &                     \\
\rowcolor[HTML]{EFEFEF} 
3.1                                             & Disconnection from requirements                                & \checkmark                                 &      & [16,42]                        \\
\rowcolor[HTML]{EFEFEF} 
3.2                                             & Grown data selection habits                                    & \checkmark                                 &                 &  [20,33]                \\
\rowcolor[HTML]{EFEFEF} 
3.3                                             & Unclear completeness criteria                                   & \checkmark                                 &              &  [49]                   \\
\rowcolor[HTML]{EFEFEF} 
3.4                                             & Unclear measure of variety                                     & \checkmark                                 & \checkmark     &   [45,50]                         \\
\textbf{4}                                       & \textbf{Overhead for monitoring solution}                      & \textbf{}                         & \textbf{\checkmark}   &                     \\
4.1                                              & Limited resources in embedded systems                          &                                   & \checkmark                &  [38]               \\
4.2                                              & Meeting timing requirements                                    &                                   & \checkmark                &                 \\
4.3                                              & Reduction of true positive rate                                &                                   & \checkmark              &                   \\
\rowcolor[HTML]{EFEFEF} 
\textbf{5}                                        & \textbf{Unclear design domain}                                 & \textbf{\checkmark}                        & \textbf{}           &              \\
\rowcolor[HTML]{EFEFEF} 
5.1                                               & Design domain depends on available data                        & \checkmark                                 &             & [6]                     \\
\rowcolor[HTML]{EFEFEF} 
5.2                                               & Uncertainty in context                                         & \checkmark                                 &            & [22]                    \\
\textbf{6}                                       & \textbf{Unsuitable safety standards}                           & \textbf{\checkmark}                        & \textbf{\checkmark}    &                    \\
6.1                                              & Focus on processes instead of technical solution            & \checkmark                                 &  \checkmark     &  [10]                          \\
6.2                                              & No guidelines for probabilistic effects in software                   &  \checkmark                                 &        &  [28,43]                        \\
6.3                                              & Safety case only through monitoring solution      &                                  &    \checkmark               & [31,46]              \\ \hline
\end{tabular}
\vspace{-10pt}
\end{table*}


==> nice_tables.tex <==
%% Nice Tables
\usepackage{booktabs}
\usepackage{array}
\usepackage{colortbl}
\usepackage{multirow}
\usepackage{longtable}


\newcolumntype{v}[1]{>{\raggedright \hspace {0pt}}p{#1}}
